Lipschitz Robustness of Finite-state Transducers

We investigate the problem of checking if a finite-state transducer is robust to uncertainty in its input. Our notion of robustness is based on the analytic notion of Lipschitz continuity --- a transducer is K-(Lipschitz) robust if the perturbation in its output is at most K times the perturbation in its input. We quantify input and output perturbation using similarity functions. We show that K-robustness is undecidable even for deterministic transducers. We identify a class of functional transducers, which admits a polynomial time automata-theoretic decision procedure for K-robustness. This class includes Mealy machines and functional letter-to-letter transducers. We also study K-robustness of nondeterministic transducers. Since a nondeterministic transducer generates a set of output words for each input word, we quantify output perturbation using set-similarity functions. We show that K-robustness of nondeterministic transducers is undecidable, even for letter-to-letter transducers. We identify a class of set-similarity functions which admit decidable K-robustness of letter-to-letter transducers.

==> app.continuous.tex <==
\ContinuityUndecidable*
\begin{proof}
\newcommand{\rep}{\overline{\mathtt{rep}}}
\newcommand{\sh}{{\overline{\mathtt{sh}}}}
\newcommand{\conf}{{\mathrm{conf}}}

We define the \emph{bounded-type} problem as follows.
Given a deterministic non-terminating Turing machine $\TM$, decide whether 
$\TM$ uses bounded space in its non-terminating computation.
The bounded-type problem is undecidable.
We show that the bounded-type problem reduces to $(\dI, \dO)$-compatibility
of a functional transducer w.r.t. given similarity functions $\dI, \dO$.

Let $\TM$ be a deterministic non-terminating Turing machine and
let $Q$ be the set of states of $\TM$. 
Assume that the alphabet of $\TM$ is $\{a,b\}$.
We define a \emph{configuration} of $\TM$ as a word
matching the regular expression $\# (a|b)^* Q (a|b)^* \#$.
We define similarity functions $\dI, \dO$ and
a functional transducer $\trans$ such that $\trans$
is $(\dI,\dO)$-compatible if and only if $\TM$ uses bounded space in 
its non-terminating computation.

The functional transducer $\trans$ is defined as follows. Its domain is
$(\rep|\sh) (\# (a|b)^* Q (a|b)^* \#)^*$, i.e., the first letter is $\rep$ or
$\sh$ and it is followed by a sequence of configurations.  The first letter
describes the mode of the transducer; $R$ stands for \emph{repeat} and
$\funcDefinedBy{\trans}(\rep C_1 C_2 \dots C_k) = C_2 \dots C_k$, whereas $S$
stands for \emph{shift} and $\funcDefinedBy{\trans}(\sh C_1 C_2 \dots C_k) =
C_1 \dots C_{k-1}$.  The similarity function $\dI$ is defined on all pairs of
words.  We put $\dI(\s,\str) = 0$ if: $\s =  \sh C_1 \dots C_k$ and $\str = \rep
C_1' \dots C_{k}'$, where $C_1$ is the initial configuration of $\TM$ and for
each $i \in \{1,\dots,k\}$, $C_i'$ is the successive (w.r.t. $\TM$)
configuration of $C_i$.  Otherwise, $\dI(\s,\str) = \infty$.  The similarity
function $\dO$ is defined on all pairs of words.  We define $\dO(\s',\str') =
0$ if $\s' \neq \str'$.  If $\s' = \str'$, $\dO(\s',\str') = 2$, when $\s'$
contains a final state of $\TM$, and $\dO(\s',\str') = 1$ otherwise. We prove
that $\TM$ uses bounded space in its non-terminating computation if and only if
$\trans$ is $(\dI,\dO)$-compatible.



$\Rightarrow$: Assume that $\TM$ uses only $N$ cells at each step of its
computation. We define automata $\autI, \autO$ computing $\dI^{\pad},
\dO^{\pad}$ on appropriate input words.  The automaton $\autI$ accepts words
consisting of \emph{aligned} configurations, i.e., words the form $(\sh \otimes
\rep) \cdot (\hat{C_1} \otimes \hat{C_1'}) \dots (\hat{C_k} \otimes
\hat{C_k'})$, where $\hat{C_i}$ (resp. $\hat{C_i'}$) results from $C_i$ (resp.
${C_i'}$) by appending $max(|C_i|,|C_i'|) - |C_i|$ (resp. $max(|C_i|,|C_i'|) -
|C_i|$) \pad-letters at the end.  The automaton $\autI$ checks whether each
pair of aligned configurations $(\hat{C_i} \otimes \hat{C_i'})$ satisfies that
$C_i$ is the successive configuration of $C_i'$ w.r.t. $\TM$. Thus, $\autI$
computes a function that $\pad$-agrees with $\dI$.

Observe that for all $\s,\str$, if $\dI(\s,\str) < \infty$ and 
$\funcDefinedBy{\trans}(\s) = \funcDefinedBy{\trans}(\str)$, then
$\funcDefinedBy{\trans}(\s)$ is a valid execution of $\TM$
starting from its second configuration. 
Assuming that each configuration is bounded by $N$,
the automaton $\autO$ works as follows. 
First, it checks whether its input $\s' \otimes \str'$
results by $\funcDefinedBy{\trans}$ from a pair $\s,\str$ such that $\autI$
evaluates $\s \otimes  \str$ to $0$. 
If this check fails, the automaton $\autO$ rejects.
If that check succeeds, the automaton $\autO$ simulates the execution of 
$\TM$ and checks whether both $\s', \str'$ coincide with the result of that simulation. 
If not, we are sure that $\s' \neq \str'$ and the value $\s' \otimes \str'$ is $0$.
If they agree with the simulation, we know that $\s' = \str'$ and the value depends
on whether they contain a final state. Clearly, $\autO$ computes a function
that $\pad$-agree with $\dO$ and it accepts the words $\s' \times \str'$
such that for some $\s, \str$, $\autI(\s \otimes \str) < \infty$,
and $\canaut$ accepts $\s \otimes \s', \str \otimes \str'$. 
Therefore, $\trans$ is $(\dI, \dO)$-compatible.

$\Leftarrow$: Suppose that there are automata $\autI, \autO$.  Consider a valid
computation of $\TM$ $C_1 \dots C_k C_{k+1}$ such that $|C_{k-1}| >
2(|\autI|+|\autO|)$.  Consider two words, $\s = \sh C_1 \dots C_k$ and $\str =
\rep C_2 \dots C_k C_{k+1}$.  Due to $(\dI, \dO)$-compatibility, $\autI$ accepts
some $\pad$-expansions $\s_{\pad}, \str_{\pad}$ or resp. $\s,\str$.  Let $p_1,
p_2$ be the starting positions of the configurations $C_{k-1}$, $C_{k}$ in
$\s_{\pad}$, respectively, and let $q$ be the position of the configuration
$C_k$ in $\str_{\pad}$. Suppose that $|p_1 - q| > |\autI|$ and assume that $p_1
< q$.  We can pump the word $\s$ between the positions $p_1$ and $q$ in
$\s_{\pad} \otimes \str_{\pad}$.  Such a pumped word would be accepted by
$\autI$, but it encodes the convolution of words $\sh C_1 \dots C_{k-1}^1 C_k$
and $\rep C_2 \dots C_{k-1}^2 C_k C_{k+1}$, where $C_{k-1}^1, C_{k-1}^2$ result
from pumping and are different than $C_{k-1}$. Such a sequence violates the
condition that $C_{k-1}^2$ is the successive configuration of $C_{k-2}$ and
$C_{k}^1$ is the successive configuration of $C_{k-1}$. Thus, the value of
$\autI$ on the pumped word should be infinite.  The case $p_1 > q$ is
symmetric. We conclude that $|p_1 - q| < |\autI|$.  However, the positions of
$C_{k-1}$, $C_{k}$ in $\s_{\pad}'$ are also $p_1, p_2$, respectively, as the
canonical automaton does not shift the letters. Also, $q$ is the position of
$C_k$ in $\str'_{\pad}$. By a similar pumping argument, we can show that $|p_2
- q| < |\autO|$. Since $|p_1 - p_2| = |C_{k-1}| > 2(|\autI|+|\autO|)$, $|p_1 -
  q| < |\autI|$ and $|p_2 - q| < |\autO|$ cannot hold simultaneously.  Thus, we
have a contradiction.  
%\qed 
\end{proof}


==> app.functional.Undedicable.tex <==
\FunctionalUndecidable*

\begin{proof}
Let $\PCPinst = \{ \lpair{v_1}{w_1}, \dots, \lpair{v_{k+1}}{w_{k+1}} \}$ be a PCP instance, where
for $i \in \{1,\dots, k\}$ we have $v_i, w_i \in \{a,b \}^*$ 
and $\lpair{v_{k+1}}{w_{k+1}} = \lpair{\$}{\$}$.

We define the transducer $\trans$ that translates indices into corresponding words
from the PCP instance $\PCPinst$. The input alphabet of the transducer is the set of indices $\{ 1,\ldots, k+1\}$, corresponding to $\PCPinst$,
marked with $L$ or $R$ denoting whether an index $i$ is translated to $v_i$, the first component of $\PCPinst$, 
or $w_i$, the second component. 
The transducer translates only indices of one kind during its run. 
That decision is made based on the first letter read. 
It is in the ``left mode'' if it translates only
indices with the marking $L$. Otherwise, it is in the ``right mode'', i.e., it translates only indices with the marking $R$.
While operating in the left mode (resp. the right mode) the transducer reads an $R$-marked letter  (resp. $L$-marked letter) it rejects. 
Finally, the last letter read by the transducer is $\lpair{k+1}{L}$ or $\lpair{k+1}{R}$.
Formally, $\trans$ is defined as follows:
\begin{enumerate}
\item the input alphabet $\Sigma$ is defined as $\{ (i, P): i \in \{1,\ldots, k+1\}, P \in \{ L, R\}\}$,
\item the output alphabet $\Gamma$ is defined as $\{ (\alpha, P): \alpha \in \{a,b,\$\}, P \in \{ L, R\}\}$,
\item the set of states $Q = \{ q_0, q_L, q_R, q_{\mathrm{acc}}, q_{\mathrm{fail}} \}$
\item the transition relation  $E$ is defined as follows
\begin{enumerate} 
\item on the beginning, the transducer reads the first letter and base on that decides
whether it will be in the ``left mode'', i.e., it will translate indices to the first components of $\PCPinst$, or 
the ``right mode'', it will translate indices to the second components of $\PCPinst$:
for every $i \in \{1, \ldots, k\}$ (without $k+1$) we have
$(q_0, \lpair{i}{L}, v_i, q_L) \in E$ and
$(q_0, \lpair{i}{R}, w_i, q_R) \in E$

\item if it in the left mode, it translates left indices $\lpair{i}{L}$, while 
it rejects upon encountering a right index:
for every $i \in \{1, \ldots, k+1\}$ we have 
$(q_L, \lpair{i}{L}, v_i, q_L) \in E$ and
$(q_L, \lpair{i}{R}, v_i, q_{\mathrm{fail}}) \in E$

\item the case for the right mode is symmetric to the left mode:
for every $i \in \{1, \ldots, k\}$ (without $k+1$) we have
$(q_R, \lpair{i}{R}, w_i, q_R) \in E$ and
$(q_R, \lpair{i}{L}, w_i, q_{\mathrm{fail}}) \in E$ 

\item to accept, the transducer has to read a letter $\lpair{k+1}{L}$ or $\lpair{k+1}{R}$, 
depending on its mode: 
$(q_L, \lpair{k+1}{L}, \$, q_{\mathrm{acc}}) \in E$ and 
$(q_L, \lpair{k+1}{R}, \$, q_{\mathrm{acc}}) \in E$.
\end{enumerate}
\item the final states $F = \{ q_{\mathrm{acc}} \}$.
\end{enumerate}

There are no transitions from the accepting state $q_{\mathrm{acc}}$, 
therefore once the transducer enters it, it has to terminate or the input will be rejected.
In  consequence,  the domain to $\trans$ is described in the following way.
We define $\Sigma_L$ (resp. $\Sigma_R$) as $\{ \lpair{i}{L} : i \in \{1,\dots, k\}\}$ 
(resp. $\{ \lpair{i}{R} : i \in \{1,\dots, k\}\}$).
Then, the following regular expression describes the domain to $\trans$:
 $\dom{\trans} = \Sigma_L^* \lpair{k+1}{L} + \Sigma_R^* \lpair{k+1}{R}$.

We define the generalized Manhattan distance such that 
$\trans$ is not robust iff $\PCPinst$ has a solution.

\noindent{\em Distance on the inputs.}
The input distance function is a generalized Manhattan distance, where 
its parameter $\diffI$ is defined as follows:
for all $P \in \{ L,R\}$ and $i,j \in \{1,\ldots, k\}$, $i \neq j$ we have
\begin{enumerate}
\item $\diffI(\lpair{i}{P},\lpair{i}{P}) = 0$,
\item $\diffI(\lpair{k+1}{P},\lpair{k+1}{P}) = 0$,  
\item $\diffI(\lpair{i}{P},\lpair{j}{P}) = \infty$,
\item $\diffI(\lpair{i}{L},\lpair{j}{R}) = \diffI(\lpair{i}{R},\lpair{j}{L}) = \infty$, 
\item $\diffI(\lpair{i}{L},\lpair{i}{R}) = \diffI(\lpair{i}{R},\lpair{i}{L}) = |v_{i}|+ |w_i|$,
\item $\diffI(\lpair{k+1}{L},\lpair{k+1}{R}) = \diffI(\lpair{k+1}{R},\lpair{k+1}{L}) = 1$,
\item $\diffI(\lpair{i}{L}, \eos) = \diffI(\eos, \lpair{i}{L}) = \infty$, 
\item $\diffI(\lpair{i}{R}, \eos) = \diffI(\eos, \lpair{i}{R}) = \infty$, and
\item $\diffI(\lpair{k+1}{R}, \eos) = \diffI(\eos, \lpair{k+1}{R}) = \infty$.
\end{enumerate}

Note that $\dI(u_1, u_2)$ is finite only if 
$\pi(u_1)$ is a prefix of $\pi(u_2)$ or vice versa.

\noindent{\em Distance on the outputs.}
The output distance function is a generalized Manhattan distance, where 
its parameter $\diffO$ is defined as follows:
for all $P \in \{ L,R\}$ and $\alpha, \beta \in \{a,b, \$\}$, $\alpha \neq \beta$ we have
\begin{enumerate}
\item $\diffO(\lpair{\alpha}{P},\lpair{\alpha}{P}) = 0$
\item $\diffO(\lpair{\alpha}{P},\lpair{\beta}{P}) = 1$
\item $\diffO(\lpair{\alpha}{L},\lpair{\alpha}{R}) = 2$
\item $\diffO(\lpair{\alpha}{L},\lpair{\beta}{R}) = 1$, and
%\item $\diffO(\lpair{\$}{L},\lpair{\$}{R}) = 3$,
\item $\diffO(\lpair{\alpha}{P},\eos) = \diffO(\eos, \lpair{\alpha}{P}) = 1$.
\end{enumerate}

Now we shall prove the final statement:
there are words $u_1, u_2 \in u_1, u_2 \in \dom{\trans}$ such that 
$\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) > \dI(u_1, u_2)$
if and only if $\PCPinst \setminus (\$,\$)$ has a solution.

$\Rightarrow$: 
For a word $u \in \{a,b\}^*$ 
%$u \in (\{1, \ldots, k+1\} \cup \{a,b,\$\})^*$ 
of length $N$, and $P \in \{ L, R\}$ we define 
$u^P$ as $\lpair{u[1]}{P} \lpair{u[2]}{P} \dots \lpair{u[n]}{P}$.
The projection $\pi$ is defined as 
 $\pi(\lpair{i_1}{P_1} \lpair{i_2}{P_2} \dots \lpair{i_n}{P_n}) = i_1 i_2 \dots i_n$, 
where $i_1,\dots,  i_n \in \{1,\ldots, k+1\}$ and $P_1, \dots, P_n \in \{ L, R\}$.


In order for $\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) > \dI(u_1, u_2)$ to hold,
$\dI(u_1, u_2)$ has to be finite. It follows that 
$\pi(u_1)$ is a prefix of $\pi(u_2)$ or vice versa. 
However, the domain of $\trans$ is \emph{prefix-free}, \ie,
$u \in \dom{\trans}$ implies that no extension of $u$ belongs to $\dom{\trans}$.
Indeed, the domain is described by the following regular expression:
 $\dom{\trans} = \Sigma_L^* \lpair{k+1}{L} + \Sigma_R^* \lpair{k+1}{R}$ and
$\lpair{k+1}{L}, \lpair{k+1}{R}$ do not belong to $\Sigma_L$ nor
$\Sigma_R$. 
In consequence,  the only $u_1, u_2 \in \dom{\trans}$ that satisfy $\dI(u_1, u_2) < \infty$
are those that satisfy $\pi(u_1) = \pi(u_2)$ and 
 $u_1, u_2 \in \Sigma_L^* \lpair{k+1}{L} \cup \Sigma_R^* \lpair{k+1}{R}$.
%
If both $u_1, u_2 \in \Sigma_L^* \lpair{k+1}{L}$ (resp. $\Sigma_R^* \lpair{k+1}{R}$), then
$u_1 = u_2$ and $\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) = \dI(u_1, u_2)$.

Consider the case $u_1 \in \Sigma_L^* \lpair{k+1}{L}$ and $u_2 \in \Sigma_R^* \lpair{k+1}{R}$ and
$\pi(u_1) = \pi(u_2)$. 
Then, there is a sequence $i_1, \ldots, i_n \in \{1, \dots, k\}$ such that
$u_1 = \lpair{i_1}{L} \lpair{i_2}{L} \dots \lpair{i_k}{L} \lpair{k+1}{L}$ 
and 
$u_2 = \lpair{i_1}{R} \lpair{i_2}{R} \dots \lpair{i_k}{R} \lpair{k+1}{R}$.
For $u_1, u_2$ the transducer produces the following outputs:
$\funcDefinedBy{\trans}(u_1) = v_{i_1}^L v_{i_2}^L \dots v_{i_n}^L \lpair{\$}{L}$ and
$\funcDefinedBy{\trans}(u_2) = w_{i_1}^R w_{i_2}^R \dots w_{i_n}^R \lpair{\$}{R}$.

Due to the definition of $\diffI$ we have $\dI(u_1, u_2) = |\funcDefinedBy{\trans}(u_1)| + |\funcDefinedBy{\trans}(u_2)|-1$.
The $-1$ component is due to the fact the $\diffI(\lpair{k+1}{L},\lpair{k+1}{R}) = 1$, 
whereas the resulting pair consists of two letters.
%%%%%%%%%%%%%%%%%%%
Now, let us examine the definition of  $\diffO$. 
The output distance $\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) = 2 \cdot \mathsf{(1)} + \mathsf{(2)} + \mathsf{(3)}$, where
\begin{itemize}
\item $\mathsf{(1)}$ is the number of positions $i$ such that 
the projections agree, \ie,
$\pi(\funcDefinedBy{\trans}(u_1))[i] = \pi(\funcDefinedBy{\trans}(u_2))[i]$, 

\item $\mathsf{(2)}$ is the number of positions, such that the projections disagree, \ie, 
$\pi(\funcDefinedBy{\trans}(u_1))[i] \neq \pi(\funcDefinedBy{\trans}(u_2))[i]$, and

\item  $\mathsf{(3)} = \abs(|\funcDefinedBy{\trans}(u_1)|,\funcDefinedBy{\trans}(u_2))$ is the length difference of $\funcDefinedBy{\trans}(u_1)$ and $\funcDefinedBy{\trans}(u_2)$. 
\end{itemize}


Observe that $\dI(u_1, u_2) = |\funcDefinedBy{\trans}(u_1)| + |\funcDefinedBy{\trans}(u_2)| = 2 \cdot (\mathsf{(1)} + \mathsf{(2)}) + \mathsf{(3)}$, therefore
$\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) > \dI(u_1, u_2)$ iff $\mathsf{(2)} = 0$.
Now, observe that if lengths of $\funcDefinedBy{\trans}(u_1)$ and $\funcDefinedBy{\trans}(u_2)$ are different,
then $(2) > 0$. Indeed, the last letter of both words is $\$$ and it occurs only once.
Assuming that $|\funcDefinedBy{\trans}(u_1)| = |\funcDefinedBy{\trans}(u_2)|$, $(2) = 0$ only if 
$\pi(\funcDefinedBy{\trans}(u_1)) = \pi(\funcDefinedBy{\trans}(u_2))$. Hence, 
$\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) > \dI(u_1, u_2)$ implies that 
$i_1, \ldots, i_n$ is the solution to $\PCPinst$.


The case $u_1 \in \Sigma_R^* \lpair{k+1}{R}$ and $u_2 \in \Sigma_L^* \lpair{k+1}{L}$ and
$\pi(u_1) = \pi(u_2)$, is symmetric.

$\Leftarrow$: Let $i_1, \dots, i_n$ be a solution to $\PCPinst$. We show that 
$\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) = \dI(u_1, u_2) +1$. Consider words
$u_1 = \lpair{i_1}{L} \lpair{i_2}{L} \dots \lpair{i_n}{L} \lpair{k+1}{L}$ and
$u_2 = \lpair{i_1}{R} \lpair{i_2}{R} \dots \lpair{i_n}{R} \lpair{k+1}{R}$.
Note that, since 
$i_1, \dots, i_n$ is a solution to $\PCPinst$,
$v_{i_1} v_{i_2} \dots v_{i_n} = w_{i_1} w_{i_2} \dots w_{i_n}$. Therefore,
%
\[\dI(u_1, u_2) = |v_{i_1} v_{i_2} \dots v_{i_n} v_{k+1}| +  |w_{i_1} w_{i_2} \dots w_{i_n} w_{k+1}|
= 2 \cdot|v_{i_1} v_{i_2} \dots v_{i_n} v_{k+1}| - 1
\]
where the $-1$ component follows from $\diffI(\lpair{k+1}{L}, \lpair{k+1}{R}) = 1$,
whereas 
%
$\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) = 2 \cdot |v_{i_1} v_{i_2} \dots v_{i_n} v_{k+1}|$
%
Thus, $\dO(\funcDefinedBy{\trans}(u_1), \funcDefinedBy{\trans}(u_2)) = \dI(u_1, u_2) +1$.
%\qed
\end{proof}


==> continuous.tex <==
\subsection{$(\dI,\dO)$-compatible transducers}

While $K$-robustness of functional transducers is undecidable in
general, we have shown in \secref{regular} that $K$-robustness of
synchronized transducers w.r.t. certain automatic similarity functions is
decidable. In what follows, we identify a more general property ---
$(\dI,\dO)$-compatibility --- which implies decidability of $K$-robustness of a
transducer $\tran$ w.r.t.  $\dI$, $\dO$.  While synchronicity is a property of
$\tran$, $(\dI,\dO)$-compatibility is a property of the triple
$(\tran,\dI,\dO)$. Moreover, while checking synchronicity is decidable
(\propref{RegularityIsDecidable}), checking $(\dI,\dO)$-compatibility is
undecidable. Despite the undecidability of checking $(\dI,\dO)$-compatibility,
we argue that this property is useful. Let us consider the following motivating
example. 

\begin{example}{\bf Skipping transducers and skipping similarity functions.}
\label{ex:SkippingMealy}
%Consider a \emph{skipping} variant of a Mealy machine defined as follows.
Given a Mealy machine $\Mea$ with input alphabet $\alphI = \{a,b\}$ and 
output alphabet $\alphO = \{a,b\}$, 
we define a transducer $\tran$, called \emph{the
skipping variant} of $\Mea$, as follows.  
The transducer $\tran$ has input alphabet $\alphI^\sk$ 
$=$ $\{ a,b\} \times \{0,1\}$ and  the same output alphabet $\alphO$ as $\Mea$.
It simulates $\Mea$ on letters $\lpair{a}{1}, \lpair{b}{1}$ while ignoring letters $\lpair{a}{0}, \lpair{b}{0}$.  
%Observe that $\tran$ is neither 
%a Mealy machine nor a synchronized transducer.  

Let $\dI, \dO$ be input and output similarity functions over $\{a,b\}^*$,
satisfying the conditions in \thmref{decidable.regular}.  Let us define a {\em
skipping} similarity function  $\dIskip$ over $(\alphI^\sk)^*$ as follows:
$\dIskip(\s^\sk,\str^\sk) = \dI(\s,\str)$, where $\s$, $\str$ $\in
\{a,b\}^*$ are obtained from $\s^\sk, \str^\sk$ by first deleting the
letters $\lpair{a}{0}, \lpair{b}{0}$ and then projecting the letters $\lpair{a}{1}, \lpair{b}{1}$ to
their first components. Observe that for every $K$, $\tran$ is $K$-robust
w.r.t. $\dIskip, \dO$ if and only if the underlying Mealy machine $\Mea$ is
$K$-robust w.r.t. $\dI, \dO$. Since $K$-robustness of $\Mea$ w.r.t.
$\dI,\dO$ is decidable (\thmref{decidable.regular}), it follows that 
$K$-robustness of $\tran$ w.r.t. $\dIskip, \dO$ is decidable . 

Let us note, however, that $\tran$ is neither a Mealy machine nor a
synchronized transducer and $\dIskip$ is not an automatic
similarity function.  Hence, we cannot use \thmref{decidable.regular} to directly decide
$K$-robustness of $\tran$ (without using $\Mea$). This, in essence, is the
motivation for defining a more general property than synchronicity that implies
decidability of $K$-robustness. Before defining this property, we explain its application
to our current example.

%In what follows, we show how to decide $K$-robustness of
%$\tran$ without explicit reference to $\Mea$. 

Let us call the letters $a$, $b$, $\lpair{a}{1}$ and $\lpair{b}{1}$ \emph{meaningful}. Given
any two input words $\s$, $\str$ over $\alphI^\sk$, we can
insert an external $\pad$ letter in both words to match up meaningful letters
in both words. Formally, two words $\s_\pad$, $\str_\pad$ over $\alphI^\sk  
\cup \{\pad\}$ (or, $\alphO \cup \{\pad\}$) are \emph{aligned} if for each $i \leq
min(|\s_\pad|,|\str_\pad|)$, $\s[i]$ is meaningful iff $\str[i]$ is meaningful.
The following example illustrates an alignment of two words: 
%if at every position of both words, either both letters are meaningful or non
%of them is. Consider the following example of alignment of two
%words:\smallskip

\noindent\begin{tikzpicture}[scale=0.75]
\tikzset{
  word/.style   = { thick,  rectangle,  minimum width=0.7cm, minimum height=0.40cm  },
  pad/.style   = { thick,  rectangle,  minimum width=0.65cm, minimum height=0.40cm }}

\begin{scope}[xshift=-9.5cm]
\node[word] at (1,0) {$\lpair{a}{1}$};
\node[word] at (2,0) {$\lpair{a}{0}$};
\node[word] at (3,0) {$\lpair{b}{0}$};
\node[word] at (4,0) {$\lpair{a}{1}$};
\node[word] at (5,0) {$\lpair{a}{1}$};

\node[word] at (1,-0.8)   {$\lpair{b}{0}$};
\node[word] at (2,-0.8) {$\lpair{b}{1}$};
\node[word] at (3,-0.8)   {$\lpair{a}{1}$};
%\node[word] at (4,-0.7) {(a,1)};
\node[word] at (0,0)   {$\s:$};
\node[word] at (0,-0.8)   {$\str:$};
\end{scope}


\node[pad] at (0,0) {$\pad$};
\node[word] at (1,0) {$\lpair{a}{1}$};
\node[word] at (2,0) {$\lpair{a}{0}$};
\node[word] at (3,0) {$\lpair{b}{0}$};
\node[word] at (4,0) {$\lpair{a}{1}$};
\node[word] at (5,0) {$\lpair{a}{1}$};

\node[word] at (0,-0.8)   {$\lpair{b}{0}$};
\node[word] at (1,-0.8) {$\lpair{b}{1}$};
\node[pad] at (2,-0.8) {$\pad$};
\node[pad] at (3,-0.8) {$\pad$};
\node[word] at (4,-0.8)   {$\lpair{a}{1}$};
\node[word] at (-1,0)   {$\s_{\pad}:$};
\node[word] at (-1,-0.8)   {$\str_{\pad}:$};

%\node[word] at (5,-0.7) {(a,1)};
\end{tikzpicture}
%\smallskip

We define a variant $\tran_{\pad}$ of $\trans$, with an input
alphabet $\alphI^\sk \cup \{ \pad\}$ and an output alphabet 
$\alphO \cup \{\pad\}$. $\trans_{\pad}$ is obtained
from $\tran$ by (a) adding a self-loop $(q,\pad,\pad,q)$ to every
state $q$ of $\tran$ and (b) changing every transition $(q,\ell,\eps,q')$
to $(q,\ell,\pad,q')$.  Observe that $\trans_{\pad}$ is a Mealy machine.  Moreover,
given a pair of aligned input words $\s$, $\str$, the corresponding pair of 
output words is also aligned.
  
As the input alphabet now includes $\pad$, we define a variant $\dIpad$ of
$\dIskip$  such that $\dIpad(\s_\pad,\str_\pad) = \dIskip(\s,\str)$ if
$\s_\pad$, $\str_\pad$ are aligned and $\s$, $\str$ are obtained from
$\s_\pad$, $\str_\pad$ by deleting all $\pad$ letters.  
%Note that
%$\dIpad(\s_\pad,\str_\pad)$ may equal $0$ for two unequal words $s_\pad$,
%$\str_\pad$. Hence $\dI^{\pad}$ is a similarity function.  
Likewise, we
define a variant $\dOpad$ of the output similarity function $\dO$.  Let
$\aut_{\dI}$, $\aut_{\dO}$ be weighted automata computing $\dI$, $\dO$,
respectively. We can construct variants $\autdIpad, \autdOpad$ of $\aut_{\dI}$,
$\aut_{\dO}$ for computing $\dIpad, \dOpad$ between aligned words. Moreover,
if $\aut_{\dI}$, $\aut_{\dO}$ satisfy the conditions of
\thmref{decidable.regular}, $\autdIpad, \autdOpad$ also 
satisfy the conditions of \thmref{decidable.regular}.

Once we have the above $\trans_{\pad}$, $\autdIpad$ and
$\autdOpad$, we can apply %the construction provided in the proof of
\thmref{decidable.regular} to decide $K$-robustness of $\tran$ w.r.t.
$\dIskip$ and $\dO$. We emphasize that this construction is
applicable because we were able to define automatic similarity
functions $\dIpad$, $\dOpad$ such that (1) $\dIpad$, $\dOpad$ 
satisfy the conditions of \thmref{decidable.regular}, (2) 
$\dIpad$, $\dOpad$ {\em agree} with $\dI$, $\dO$, respectively 
on all aligned words, and (3) for any
two words $\s$, $\str$ over $\alphI^\sk$ with $\dIskip(\s,\str) < \infty$, there exist 
corresponding aligned words $\s_\pad$, $\str_\pad$ over $\alphI^\sk \cup \{
\pad\}$ such that $(\s_\pad,\str_\pad) \in \dom{\dIpad}$ 
and $(\funcDefinedBy{\tran_\pad}(\s_\pad), \funcDefinedBy{\tran_\pad}(\str_\pad)) \in \dom{\dOpad}$.
\end{example}
\noindent In what follows, we generalize the above principle.\\ 
%The construction from Example \ref{ex:SkippingMealy} is an instance of
%a general technique explained below. 

\noindent {\bf $\pad$-expansions.}
Let us denote by $\alphI_\pad$ the alphabet $\alphI \cup \{\pad\}$. 
Let $\s$ be a word in $\alphI^*$. We say a word $\s_\pad$ 
is a $\pad$-expansion of $\s$ iff $\s_\pad \in (\alphIPad)^*$ 
and the word obtained by removing all $\pad$
letters from $\s_\pad$
%, denoted $\pi(\s_\pad)$, 
is $\s$.
\medskip

\noindent {\bf $\pad$-agreement.} Let $\dI$ be a similarity function over $\alphI^*$. 
A function $\dIpad$ \emph{$\pad$-agrees} with $\dI$ iff for all 
words $\s,\str \in \alphI^*$, for all their $\pad$-expansions $\s_{\pad}, \str_{\pad}$,
$(\s_{\pad}, \str_{\pad}) \in \dom{\dIpad}$ $\Rightarrow$ 
$\dIpad(\s_{\pad}, \str_{\pad}) = \dI(\s,\str)$.
\medskip

\noindent {\bf Canonical transducer.}
Given a functional transducer $\tran$ with $\funcDefinedBy{\tran} \subseteq \alphI^* \times 
\alphO^*$, we present a constructive definition for a canonical transducer
 $\cantran$ with $\funcDefinedBy{\cantran} \subseteq \alphI_{\pad}^* \times 
\alphO_{\pad}^*$. The transducer $\cantran$ is obtained 
by substituting 
\begin{compactenum}
%\item substitute every transition $(q,a,\out,q')$ in $\trans$ with $|\out| = 1$ 
%with a transition $(q,\, a \otimes \out, \, q')$ in $\canaut$,  
\item every transition $(q, a, \out, q')$ in
$\tran$ with $|\out| \geq 2$ by a path in $\cantran$ of the form: 
%$(q,a, \out[1],\, q^{1}), (q^{1}, \, \pad \otimes \out[2], \, q^2), \ldots, (q^{n-1},\, \pad \otimes \out[n], \, q')$,
$(q,a, \out[1], q^{1}), (q^{1}, \pad,\out[2], q^2), \ldots, (q^{n-1}, \pad, \out[n], q')$,
where $n = |\out|$ and $q^{1},\ldots,q^{n-1}$ are new states not in $\trans$, and 
\item every transition $(q, a, \eps, q')$ in $\tran$ by
$(q, a, \pad, q')$.
\end{compactenum}
The canonical transducer $\cantran$ for $\tran$ is a functional letter-to-letter transducer, 
and therefore, a synchronized transducer.
Note that for all $\s \in \alphI^*, \s' \in \alphO^*$,
$\funcDefinedBy{\trans}(\s) = \s'$ iff there
are $\pad$-expansions $\s_\pad$, $\s'_\pad$ of $\s$, $\s'$ such
that $\funcDefinedBy{\cantran}(\s_\pad) = \s'_{\pad}$.
%\smallskip
%\medskip

\begin{definition}[\bf $(\dI,\dO)$-Compatibility]
Given similarity functions $\dI, \dO$, 
we say that a functional transducer $\tran$  is \emph{$(\dI, \dO)$-compatible}
iff there are automatic similarity functions $\dIpad, \dOpad$ satisfying the following conditions: 
\begin{compactenum}[(C1)]
\item there is a linear value function $f$ 
%such that %$f$-weighted automata $\autI, \autO$
such that $\dIpad$ is computed by an $f$-weighted automaton and
$\dOpad$ is computed by a functional $f$-weighted automaton, %that computes $\dOpad$,
\label{cont-cond1}
\item $\dIpad$, $\dOpad$ $\pad$-agree with $\dI$, $\dO$, respectively, and 
\label{cont-cond2}
\item for all $\s,\str \in \dom{\tran}$ with  $\dI(\s,\str) < \infty$ there exist 
$\s_\pad,\str_\pad \in \dom{\cantran}$ such that
$\s_\pad,\str_\pad$ are $\pad$-expansions of $\s,\str$, 
 $(\s_\pad,\str_\pad) \in \dom{\dIpad}$, and
% \str_\pad \in \dom{\cantran}$, and
$(\funcDefinedBy{\cantran}(\s_\pad), \funcDefinedBy{\cantran}(\str_\pad)) \in \dom{\dOpad}$.
\label{cont-cond3}
\end{compactenum}
\end{definition}

\begin{theorem}
\label{t:cont}
\label{thm:decidable.cont}
Given similarity functions $\dI, \dO$ and a $(\dI, \dO)$-compatible
transducer $\tran$, $K$-robustness
of $\tran$ is decidable.
\end{theorem}

\begin{proof}
The definition of $(\dI, \dO)$-compatibility implies that
$K$-robustness of $(\dI, \dO)$-compatible $\tran$ 
can be reduced to $K$-robustness of the canonical transducer $\cantran$ for $\tran$
w.r.t. automatic similarity functions $\dI^{\pad}, \dO^{\pad}$. 
Indeed, consider similarity functions $\dIpad, \dOpad$ from the definition of 
$(\dI, \dO)$-compatibility of $\trans$. 
Condition (C2) of $(\dI, \dO)$-compatibility implies that
if $\trans$ is $K$-robust w.r.t. $\dI, \dO$, then 
$\cantran$ is $K$-robust w.r.t. $\dIpad, \dOpad$. 
Condition (C3) implies the converse. Thus, 
$\cantran$ is $K$-robust w.r.t. $\dIpad, \dOpad$ iff
$\trans$ is $K$-robust w.r.t. $\dI, \dO$. 
Finally, synchronicity of $\cantran$ and
Condition (C1) of $(\dI, \dO)$-compatibility imply that 
 $K$-robustness of $\cantran$ w.r.t. $\dIpad, \dOpad$  can be decided 
using \thmref{decidable.regular}.
\qed
\end{proof}

As mentioned already, although $(\dI, \dO)$-compatibility 
implies decidability of $K$-robustness, it is itself 
an undecidable property. 

\begin{restatable}{proposition}{ContinuityUndecidable}
\label{p:cont-undecidable}
Given similarity functions $\dI, \dO$ and a transducer $\tran$,
checking whether $\tran$ is $(\dI, \dO)$-compatible is undecidable.
\end{restatable}
\noindent\emph{Proof sketch.} 
Given a Turing machine $\TM$,  
we define a similarity function on inputs $\dI$ and a transducer $\tran$
such that $\s,\str \in \dom{\tran}$, $\dI(\s,\str) < \infty$ and 
$\funcDefinedBy{\trans}(\s) = \funcDefinedBy{\trans}(\str)$ iff
$\s$ is a sequence of consecutive configurations of $\TM$.
Such a transducer $\tran$ is $(\dI, \dO)$-compatible iff 
$\TM$ is equivalent to a finite-state automaton. Indeed, from automata 
for $\dI, \dO$ and the canonical transducer for $\tran$, one
can construct an automaton simulating $\TM$. 
Since checking if a Turing machine is equivalent to a finite-state automaton 
is undecidable, checking $(\dI, \dO)$-compatibility is undecidable.



